Compositor: Bottom-up Clustering and Compositing for Robust Part and Object Segmentation

In this work, we present a robust approach for joint part and object segmentation. Specifically, we reformulate object and part segmentation as an optimization problem and build a hierarchical feature representation including pixel, part, and object-level embeddings to solve it in a bottom-up clustering manner. Pixels are grouped into several clusters where the part-level embeddings serve as cluster centers. Afterwards, object masks are obtained by compositing the part proposals. This bottom-up interaction is shown to be effective in integrating information from lower semantic levels to higher semantic levels. Based on that, our novel approach Compositor produces part and object segmentation masks simultaneously while improving the mask quality. Compositor achieves state-of-the-art performance on PartImageNet and Pascal-Part by outperforming previous methods by around 0.9% and 1.3% on PartImageNet, 0.4% and 1.7% on Pascal-Part in terms of part and object mIoU and demonstrates better robustness against occlusion by around 4.4% and 7.1% on part and object respectively. Code will be available at https://github.com/TACJu/Compositor.

==> 04_method_old.tex <==
\section{Method}

\alan{\section*{Alan's Formulation of the Methods}}

\subsection*{Formulating the model for part detection only}

First we describe the model for detecting parts only (i.e. Qihang's model). This requires: (i)  specifying how the algorithm is applied to an input image (after all the parameters of the model have been learnt), (ii) how we learn the parameters of the model.We start by describing the model after it has been learned. 

The input feature vectors $\{f_i(I,\theta): i \in D\}$ are computed from an input image $I$ defined over a domain $D$ by a deep network with learnt  parameters $\theta$. The output is a decomposition of the image into a subset of regions where each region has a class label (e.g., part-A, part-B, background). Formally, the algorithm decomposes $D$ into disjoint regions $\{D_a: a \in A\}$, such that $\bigcup _a D_a = D$ and $ D_a \bigcap D_b = \empty$ for all $a \neq b$, Each region has 
 has a class label $c_a \in \{1,...,K\}$ corresponding to object parts or to background regions. The algorithm predicts the decomposition by using the K-means algorithm to minimize the cost function 
 
 \begin{equation} E(W,P) = \sum _{ia} W_{ia} sim(F_i,P_a) + T \sum _{ia} W_{ia} \log W_{ia},\ \ \sum _a W_{ia} =1, \ \forall \end{equation} 
 This estimates the part-centroids $\{P_a\}$ and the assignments $\{W_{ia}\}$ between the pixels $i \in D$ and the part regions $D_a$. This formulation assumes that the $\{F_i\}$ are generated by a mixture of Gaussians (with variance specified by $T$) centered on the $\{P_a\}$. The assignments are soft so that each $W_{ia} \in (0,1)$ (the assignments become hard in the limit as $T \mapsto 0$). 
 
 The class $c_a$ of the region $D_a$ is predicted by a multi-layer perceptron $c_a = g(P_a; \phi)$ with learnable parameters  $\phi$. In summary, the prediction for an image $I$ has regions $D_a$ specified by the $W_{ia}$, with centroid $P_a$, and class $g(P_a; \phi)$.
 
 This formulation assumes that we can learn feature vectors $\{f_i(I;\theta)\}$ which are similar within each part region $D_a$ and hence are close to the estimated $P_a$. These are feature embeddings because they must capture the semantic properties of the parts and not just intensity properties. This is plausible for the part regions but seems much less likely for the background region (the model assumes that some regions of the image are object parts and other regions are background).
 
 Inferring $P$ and $W$ can be done by minimizing $E(W,P)$ with respect to $P$ and $W$ respectively. But $E(W,P)$ is a non-convex energy function so good initialization is needed. One possibility, see next paragraph, is to find good initialization for each part.
 
 For each images we estimate the $P$ and $W$ by the following update rules:
\begin{equation} W_{ia} = {{\exp (f_i - P_a)^2/T}\over{\sum _b \exp (f_i - P_b)^2/T}} \ \ P_a = \sum _i W_{ia} f_i,\end{equation}
\noindent which are minimizing $E(P,W)$ with respect to $W$ and $P$ respectively. ({\it Note: this is quadratic -- what if the $P$ and $f$ are normalized?}). 
 
 An important question is whether different instance of the same part has similar feature vectors. More specifically, we should study the set  $S_k = \{P_a: \ c_a =k\}$ obtained for the same part $k$ from all images. (Where the $P_a$ are the part centroids which correspond to part $k$ from the set of images $\{I^{n}: n=1,...N\}$). This is being studied. It is plausible ffor the part regions that $S_k$ corresponds to tight cluster in feature space with mean ${\hat P}_k$ (this is being checked) for the part regions (or we may be able to modify the learning to encourage this). But it probably is not correct for the background regions (and maybe the model should be modified?).
 
Now we will discuss how the parameters $\theta, \phi$ of the model are learnt from a set of images $\{I^{t}: t=1,...,N\}$ with annotated regions and classes $\{D_a^n, c_a^n\}$. We need to learn feature vectors which are very similar within each part instance (and possible also between different instances of the same part). 

The loss function for learning requires comparing the predictions of the model with the groundtruth. This can be done per-pixel, as is standard for visual tasks like semantic segmentation, but this is known to be problematic because it ignores the context. Instead, following Huiyu (and UIUC people), we formulate this as a matching problem between the predicted regions, and their predicted classes, and the groundtruth regions and classes.

\begin{equation} E(\{V^t\}: \theta, \phi) = \sum _t \sum _{a,b} V_{a,b}^t sim(D_{a}^t(\theta, I^t),D_b^t) sim (c_a(\theta, I^t), k_b^t). \ \ \sum _a V^t_{ia} = 1 \ \forall i \ \ \sum _i V^t_{ia} = 1 \ \forall a.\end{equation}

\alan{Old stuff after this.}
 

which take values in feature space, and which correspond to subregions/masks of the image by binary-valued correspondence variables $W_{ia}$ which assign each pixel $i$ to one of the part-centroids $a$. These part-centroids and their correspondences are computed from the input feature vectors $F_i(I,\theta)$ by k-means clustering using a few iterations to minimize the following function by coordinate descent (how initialized?) \ju{Gaussian: N(0,1)} \alan{During learning, the algorithm is modified to have a residual connection and a learnable parameter. Alan thinks the residual connection is simply a modification of the M-step in EM (instead of minimizing wrt $P$ the algorithm does an iteration of steepest descent) and the learnable parameter does not do much (according to Qihang)}. 

\alan{The Hungarian algorithm also has this type of instability during learning (according to Qihang) so maybe it could be replcaed by a more stable algorithm, like the neural netwrok algorithms that Alan worked on in the 1990's. The Hungarian algorithm originated in Huiyu's work, so ask him about it,}

\begin{equation} E(W,P) = \sum _{is} W_{ia} sim(F_i,P_a),\ \ \sum _a W_{ia} =1 \ \forall i.\end{equation} 
\noindent here $sim(.,.)$ is a similarity measure, e.g., the dot product of the (normalized) feature vectors $F_i$ and $P_a$. \alan{Qihang says that this similarity measure can include some learnable paramters (e.g., linear projection or even MLP).}

The second variables are the predicted classes for each region/mask. This is specified by $c_a = g(P_a,\phi)$ where $g(.,.)$ is a multilayer perceptron specified by parameters $\phi$ which will also be learnt. 



In summary, the $\{P_a, W_{ia}\}$ will specify the masks/regions and the $\{c_a\}$ will predict the classes. The inference algorithm requires computing the $\{F_i\}$, iterations of k-means to compute $\{P,W\}$ followed by an MLP to compute the $\{c\}$. Can this be done more simply by using k-nearest neighbour. \alan{Are the centroids similar for different instances of the parts? If so, this could be exploited.} 

Now we discuss the learning. Alan argues that we learn the parameters $\theta, \phi$ (and other parameters like in the similarity measure) but we do not learn the $P's$ or the $W$'s  because they are latent variables which are estimated separately for each training image. 

During learning, we index the images by a superscript variable $t$. We need to have a similarity measure between the ground-truth masks $\{m_b^t, k_b^t\}$, where the $m_b^t$ specify the pixels in region/mask $b^t$ and $k_b^t$ is the class label, for image $I^t$.

\alan{Why use the linear assignment formulation? The simplest formulation would be to compare the predictions of the algorithm to the groundtruth pixel by pixel. But this is a local measure of similarity (which has known limitations) and, as described in Huiyu's paper (and the UIUC work), perhaps it is better to compare the mask and class predictions directly.}

This can be formulated as a correspondence problem with energy:

\begin{equation} E(\{V^t\}: \theta, \phi) = \sum _t \sum _{a,b} V_{a,b}^t sim(W_{ia}^t(\theta, I^t),m_b^t) sim (c_a(\theta, I^t), k_b^t). \ \ \sum _a V^t_{ia} = 1 \ \forall i \ \ \sum _i V^t_{ia} = 1 \ \forall a.\end{equation}
\alan{Alan argues that the $P$'s are not learnable because it is a latent variable which is estimated for each image. From the input image $I^t$ the algorithm estimates the features $F(I^t;\theta)$, from these it estimates the $P^t$ and the $W^t$.}

\alan{New material} The equation above imposes 1-1 correspondence between the predictions of the model and the groundtruth. This is natural for Qihang's work on panoptic segmentation (and Huiyu's earlier work) and the minimization can be done by the Hungarian algorithm. But for Ju's problem our ground truth will have $H^t$ object parts annotated (as foreground) and $1$ background region for image $I^t$. The K-means algorithm, however, will output $K$ regions within which the feature vectors are roughly constant.  It is unrealistic that we can learn features vectors which are roughly constant within the entire background region. Therefore it seems more realistic to model the background in terms of $K-H$ subregions within which the feature vectors are roughly constant. We can use the same energy formulation above, but we need to modify the constraints. Each predicted subregion $\{i=1,...,K\}$ is required to match one of the $H$ part regions $\{a=1,...,H\}$ or the background region with index $a=0$. This gives a $K x (H+1)$ matrix with components $V_{ia}$ obeying constraints $\sum _a V_{ia} = 1,\ \forall i$ and constraints $\sum _i V_{ia} =1 \ a=1,...,H$ and $\sum _i V_{ia} = K-H, \ a=0$. In other words, each of the parts match one of the groundtruth regions and the background regions is decomposed into  $K-H$ subregions.

This energy function cannot be minimized by the Hungarian algorithm. But we can formulate a relaxed version of the problem by adding an entropy term $T \sum V_{ia} \log V_{ia}$ and allowing each $V_{ia}$ to take continuous values in the range $[0,1]$. We know impose the constraints by introducing lagrange multiplier terms $\sum _{i=1}^K Q_i \{\sum _a V_{ia} -1\}$, $\sum _{a=1}^H P_a \{ \sum _{i} V_{ia} - 1\}$, and $P_0 \{\sum _i V_{ia} - (K-H)\}.$

Note that $E_{rel}[V;Q,P] $ which equals $E{V}$ plus these linear constraints and the added entropy term is a convex function of $V$ and  has a unique global minimum. It can be shown (Kosowsky and Yuille 1993) that the minimum of $E_{rel}[V;P,Q]$for small $T$ is close to the solution for the non-relaxed original problem (strictly speaking, we proved this for the special 1-1 correspondence case).

There are a range of algorithms that can minimize $E_{rel}[V:P,Q]$. The easiest is to use primal duality theory. This requires minimizing $E_{rel}[V:P,Q]$ to solve for $V(P,Q)$ as a function of $P,Q$ and substitute to obtain the dual energy $E_{dual}[P,Q] = E_{rel}[V(P,Q),P,Q]$ (these steps can be done analytically). Next we maximize $E_{dual}[P,Q]$ with respect to $P$ and $Q$ alternatively (these update equations are easy to derive). In the special case of 1-1 matching this algorithm corresponds to Sinkhorn's algorithm (Kosowsky and Yuille 1993). For the new linear constraints, we obtain an algorithm which is very similar (Ju can work out the details by doing the steps discussed above -- and then check them with Alan).

Note there are variants of this formulation. We could, for example, try to make the centroids different between different k-means clusters (e.g., add a contrastive loss term). We can also try to penalize the centroids for each part to differ between instances.

\alan{This formulation is too simple. Instead we have a sum over levels/layers/stages with explicit $P$ values in each. At the first stage, we use $P_{init}$  which is learnable. Alternatively, we could have a quadratic penalty between $P_{init}$ and the $P$ computed from the K-means. This gives good initialization but also encourages the $P$ values to be similar for different instances of the same part-type.}
Here $sim(W_{ia}^t(\theta),m_b^t)$ is a measure of similarity between the groundtruth mask $m_a^t$ and the predicted mask $W_{ia}^t$, and $sim(c_a(I^t, \theta),k_b^t)$ is a cross-entropy loss (are there any learnable parameters here?). This mininization requires that that the number of predicted masks and the number of groundtruth masks is the same (which can be fixed by padding). The minimization can be done by the Hungarian algorithm.

\alan{Are the $P$ similar for different images but for the same parts. I.e. for dog-torso are the $P$ very similar for different images? CAn this be checked by Ju/Intern.}

\alan{Questions: What types of errors do the part-masks make? Do they always detect the correct parts? Or do they miss some? Are their errors due to failures to predict the parts accurately? My point is that the model does part detection and part localization -- and both these tasks can be evaluated separately. Can Ju/intern check this out and see what types of errors are made.}

\alan{Error Analysis: New Material Starts here}

The current evaluation measures give performance of $0.65$ fr all part-types. This is computed by predicting the parts (their types and the image regions they cover) and computing the overlap with the ground truth parts. For a specific image we have $K$ predicted regions $\{(D^P_k,\tau ^P_k,P^P_k): k=1,..,K\}$ where $D^P_k$ is the image region, $\tau _k$ is the predicted part-type, and $P_k$ is the mean feature vector. We also have $H$ groundtruth regions $\{(D^{GT}_h, \tau ^{GT} _h, P_h^{GT}); h=1,..H\}$ with $H<K$. For each part-type $\tau$ we define a measure $M(.,.)$ of similarity between the predicted regions with type $\tau$ --- $\bigcup _{k, \tau ^P_k= \tau} D^P_k$ -- and the groundtruth regions with the same type $\tau$ $\bigcup _{k, \tau ^{GT}_h= \tau} D^{GT}_h$. A typical similarity measure is the IOU between the regions. To get the total measure we sum over all possible part-types $\tau$. This give the mIOU (which we sum over all testing images). For each image, we have an error measure

$$ \sum_{\tau} M(\bigcup _{k, \tau ^P_k= \tau} D^P_k, \bigcup _{k, \tau ^{GT}_h= \tau} D^{GT}_h).$$

This is the measured used in the paper ({\it Alan thinks, Ju should check}). In order to understand performance better, and hence improve the model, we need more detailed analysis. 

Here are some examples: (I) How often do the predictions have false-negatives and fail to predict a part-type? False-negatives. I.e. for part-type $\tau ^{GT}_h$ there is {\it either} no predicted part-type $\tau ^P_k = \tau ^{GT}_h, \ \forall k$ {\it or} there is a predicted part-type $\tau ^P_k = \tau ^{GT}_h$ but there is no overlap between the two regions  $D^{GT}_h \bigcap D^P_k = \emptyset$. (II) As a variant of the false-negatives, if we predict the region correctly but {\it have the wrong part-type}  -- i.e. $D^{GT}_h \bigcap D^P_k \neq  \emptyset$ but $\tau ^{PP}_k \neq \tau _h^{GT}$. How often does this happen? (III) How often do we make false-positive predictions and predict part-types which are not in the image-- i.e. we have predicted type regions $\{D^P_k, \tau ^P_k, P^P_k\}$ but there is no groundtruth region with type $\tau ^P_k$. 

It is important to understand if these types of errors occur and how often. Because we can modify the algorithms to correct them,  if we exploit use of  object-level knowledge (i.e. that an object consists of a set of part-types). In each image there will be only one object and its parts will be close to each (they should touch) and there will be constraints on where the parts can be relative to each other, but these constraints are complex and should be left for future work (I have ideas about how to enforce them). I sketch an approach here: (I) To  exploit object knowledge, we need to predict the object class from the predicted part-types.To do this the  predicted part-types can give votes for the identity of the object in the image (the votes could be weighted by the specific part-type, e.g., the part-type for the head of an object should probably have a strong weight) and these votes could be estimated by how frequently the part-type correctly predicts the object class). (II) Assuming we have a predicted object class, then we can decrease the false-positives by removing part-types which are not consistent with the predicted object class. We can also use other cues, e.g., remove false-positive regions which are not spatially contiguous. (II) For mistakes where we predict the correct region, but wrong part-type, we have see which part-types can be easily confused and see if changing the part-type (to one consistent with the predicted object) can improve performance. (III) How can we improve the detection of false negatives, where we fail to detect the part and there is no proposed part anywhere near it? This may be possible if the feature vectors of the part-types are similar between different images, see next paragraph.

For each part-type, and each instance  $\mu$, we will get a feature vector $P_{\tau}^{\mu}$ (the average of the feature vectors within each part regions. This gives a set $\{ P_{\tau}^{\mu}: \mu\}$ of feature vectors. We conjecture, that this set is tight in the sense that all the feature vectors are very similar to each other. And ideally different to the feature vectors for the other types. So if we have predicted an object part, but suspect that some parts are missing, then we could look for regions in the image where the feature vectors are similar to the feature vectors of the missing types. 

In the analysis above, I've ignored cases where the algorithm detects the part-type correctly but the region prediction (overlap) is small (which will cause big errors). The same analysis described above can be done if we put a threshold on the overlap between the predicted part region and the ground truth part region -- i.e., by requiring overlap of over $0.3$. To get some understanding, we could plot a histogram of the best region overlap for all the detected object parts. 

\alan{Error Analysis: New Material Starts here}


\alan{Note: Ju says that the initializations of the $\{P\}$ (and $\{O\}$) are learnable. "Regarding the important distinction, I think there might be some misunderstandings in how I present my thoughts. P and O are first initialized with N(0,1), however, their initialized weights are learnable instead of fixed as N(0,1). In this case, P and O will gradually be learned through the whole dataset to obtain a good initialization weight followed by being estimated based on each image differently and obtain the final P' and O' to compute the prediction mask. As the initial weights are gradually learned, so I call P and O also learnable parameters."}
 
\alan{With occlusion -- how much? -- part detection may drop by about by about 15 percent. Need more details}
    
\subsection*{The model with parts and whole objects}

\alan{When the part-masks are detected then this means that we know the object class. Ju says this isn't correct because the parts are annotated on super-classes. We would need to convert them to fine-grained classes if we want (which is possible).So current formulation means we have to search over the object classes. }

We introduce $O$ variables -- 

The key idea of compositor is to combine the parts to form the whole object. This is a difficult task and historically has been formulated as a parsing tasks and using  AND-OR graphs. But AND-OR graphs are challenging because we have to specify: (i) which combinations of parts can occur, (ii) an algorithm for searching over the possible part combinations. We conjecture that, similar to NLP, we may be able to obtain parsing results using  a simpler method using semantic features which can then be interpreted/checked using AND-OR graphs, see later section. 

\alan{I'm not sure I understand what is done. And I'm not sure it is the best formulation. I describe what I think is happening.}

We introduce new variables which represent semantic features of objects $\{O_l\}$ and their assignments $W_{li}$ to the image pixels $i$ -- but maybe the assignments are to the parts $W_{la}$? The intuition seems to be that for each image we estimate a set of part-masks (proposals) $\{P^a,W^a\}$ and select those part-masks which are similar to the semantic features $O$ of the object.

\alan{I do not understand how this is done in the paper. There are a set of update equations (13-15) which, I am told, correspond to the third loss term in equation (3). But this is inconsistent because equations (13-15) uses a sigmoid function. Also equations (13-15) do not explain what it means to say that $P$ is selected. How many $O$'s are there? Are they learnt? Or estimated for each image.}

At present, if we run equations (13-15) it seems that we select part-masks which most similar to each other (equivalently all the $P$'s are similar to a single $O$.

This seems to ignore a lot of information. When we are learning we know the mask of the entire object and we should be able to exploit this.


But this means we have to estimate $O$ for each images. How do we do this? One possibility is for the $O$'s to be estimated from the  input feature vectors $F_i$ by a deep network $O= h(F;\psi)$ where $\psi$ parameterizes the deep network. Another, which Ju says is used, is that the $O$'s are estimated from the part centroids, i.e. $O= h(P;\psi)$. The functional form is described through equation \ref{formula:object_update} (13-15). And yes we currently have only one object and one background centroid in each image. \alan{No, equations 13-15 do not answer my question. I'm unsure why the $0$'s are computed from the $P$'s and not from the $F$'s.}.

To match the part-proposals (the output of the previous section) to the object we minimize an energy function:
\begin{equation} \sum _a V_a sim(W_{ia}(\theta),O_b).\end{equation}
Here the $V_a$ are binary-valued. $V_a=1$ means that part-proposal $a$ is selected to be part of the object. The similarity measure selects parts whose feature vectors are similar to those of the object. 

In order to learn the deep network parameters $\theta, \phi, \psi$ we need an additional loss function. Presumably we formulate this by finding the correspondence between the object-centroids/masks and the ground-truth object masks (what about the class labels?). But we also need to have terms like $\sum _a V_a sim(W_{ia}(\theta),O_b)$ to ensure that the centroid-features of the parts and similar to the centroid-features of the objects. \alan{Is this right? What are the details?}
\ju{Similar to the above equation, I think we should have \begin{equation} E(V: \theta,\phi,\psi) = \sum _{a,b} X_{a,b} sim(X_{ia}(\theta),m_b) sim (d_a(\theta), k_b). \ \ \sum _a X_{ia} = 1 \ \forall i \ \ \sum _i X_{ia} = 1 \ \forall a.\end{equation} here, again that $O$ is also learnable and should be incorporated. Currently I think we don't have explicit loss term to ensure the centroid-features of the parts and similar to the centroid-features of the objects are similar.} \alan{I don't understand the reason for having variables $X_{ia}$. It would make sense if you have several objects in the image. But you only have one object and the rest of the image is background. So I think using $V_a$ is sufficient.} \alan{Surely $O$, like $P$, is not learning. These variables are estimated during infernece. The parameters $\theta, \phi, \psi$.}

\alan{But it seems that we could also have an energy term which enforces that the part-masks combine to fit the object-masks.}
\ju{I think this relates to the above point, like if we find a way to combine the part masks to fit the object masks then we can also have a term to penalize the distance between part centroids and object centroids.} \alan{I don't think this is difficult.}

In Ju's system, alan thinks that all the parameters $\theta, \phi, \psi$ \ju{should be $\theta, \phi, \psi, P, Q$} \alan{I disagree -- I think $P,O$ are estimated for each image and are not learnt.} are trained jointly together, which is consistent. {\it But} during inference the $\{P\}$ are only estimated by minimizing the energy in the previous section. It would be theoretically better to perform inference by minimizing all the energy functions -- even if we start by minimizing the first energy function for the $\{P\}$ first and then refine the $\{P\}$ in a later stage.
\ju{As $Q$ is estimated from $P$, actually $\phi$ and P should also get optimized when minimizing the latter energy functions, am I right?} \alan{We need to discuss}.

\alan{Simple experiment -- find the best parts -- and then combine them together to find the whole object. Ju/Intern should do this.}

\alan{More interesting if sometimes we fail to detect some parts -- e.g., small parts -- but detecting the objects enables us to discover the small parts.}

\subsection*{What Next? How to do top-down? What about AND-OR graphs}

There are open questions in the previous section and probably natural ways to improve the algorithm (or to correct Alan's misunderstandings). 

The method can be tested when there is occlusion -- artifically added like in the compnet papers -- to see if the algorithms here can generalize to out-of-distribution data.

The method could also be applied to human parsing because there is a lot of interest in this.

What about top-down? Alan thinks that top-down means that we have an object model that knows about the parts and their possible relative configurations (where parts can be relative to each other). This is like specifying an AND-OR graph for the object. This is very difficult without a lot of work. But perhaps we could use Ju's model as a bottom-up techniques that makes proposals for object parts that can be checked for consistency and refined? What type of object model -- is a 3D SAMP model possible? (But we don't have many of them).

How does Ju's approach relate to classical methods for composing objects together from their parts? The main idea here is that (following Huiyu, Qihang) we have magic-features. Standard image features captured properties of the image intensities only. But magic-features seem able to capture the semantic structure of objects as well (e.g., the magic features are similar throughout all parts of an object, even if the object is inhomogeneous and hence would have different image-based features). These magic-features seem too good to be true -- but they seem to make it possible to do tasks that are very hard to do. Can we relate the results of the magic features to the findings of Chris Manning about NLP grammars being related to deep network features?

What happens if we train these types of models without class labels? This seems similar to super-pixels. Can we perform edge/boundary detection using them? Can we detect new objects that we havn't annotated?


\alan{Alan stops here}

In this section, we first provide a view that regards the object segmentation problem as an optimization problem of learning a feature vector as a centroid for grouping corresponding pixels. Meanwhile, we introduce a hierarchical representation to tackle the problem from part to whole. Afterwards, we illustrate the proposed Compositor, which clusters pixel embedding to part embedding and further composites part embedding to obtain object embedding. In the end, we provide the details of the model instantiation.

\subsection{Segmentation as Clustering and Compositing}

Segmentation aims to segment the image $\mathbf{I} \in \mathbb{R}^{H \times W \times 3}$ into a set of masks with associated labels: 
\begin{equation}
\{y_i\}_{i=1}^M = \{(m_i, c_i)\}_{i=1}^M \,,
\end{equation}
where $m_i \in {\{0,1\}}^{H \times W}$ indicates whether a pixel belongs to mask $m_i$ and $c_i$ denotes the ground truth class label of mask $m_i$. $M$ is the number of different labels (masks) existing in the image.

Two mainstream methods exist to tackle this problem. One directly gives the a per-pixel prediction with a prediction head in FCN manner~\cite{long2015fully, chen2017deeplab}. Another one, inspired by the transformers~\cite{vaswani2017attention}, proposes to disentangle the problem into class-agnostic mask segmentation and mask classification~\cite{carion2020end, wang2021max, cheng2021per}. In this paper, we present a more general view of the problem, by considering the task of segmentation is essentially the same as learning a feature embedding, which can serve as a centroid to group the corresponding pixels together and thus formulates a mask. Specifically, we reformulate the energy function to minimize for part and object segmentation during training as follows:
\alan{First equation should be $\mathbf{F} = f(\mathbf{I},\theta)$.}
\begin{align}
    \centering
    \mathbf{F}, \mathbf{P}, \mathbf{O} &= f(\mathbf{I};\theta), \\
    \mathrm{minimize}~ \alpha \times \sum_{i=1}^{HW}\sum_{j=1}^{N}V_{ij}\cdot\mathrm{Dis}(\mathbf{F}_i,\mathbf{P}_j) &+ \beta \times \sum_{i=1}^{HW}\sum_{k=1}^{M}V_{ik}\cdot\mathrm{Dis}(\mathbf{F}_i,\mathbf{O}_k) + \gamma \times \sum_{j=1}^{N}\sum_{k=1}^{M}V_{jk}\cdot\mathrm{Dis}(\mathbf{P}_j,\mathbf{O}_k),
    \label{formula:opt_goal}
\end{align}
% with respect to
\alan{What are we minimizing? What are the variables? The $V_{ij}, V_{ik}, V_{jk}$ are groundtruth. Really we should have $\sum{_m}$ where $m$ indexes the images and the $V$'s should have an $m$ index. We are minimizing the parameters $\theta$ of the network and the $P$'s and $O$'s.  What algorithm are we using to minimize this Ju says we only need one of the second and third terms (probably we don't need the second term?). Surely equation (2) is incorrect. It should be $F=f(I:\theta)$. But then what are $P$ and $O$? Are these extra variables like the $V$'s?. Each feature vector $F_i$ is assigned to only one $P_j$. For the third term, some $P_j$ correspond to the object $O_k$ but others do not. In practice, each part is selected or rejected independently. Estimate feature vector $O_k$ for the object. $k$ takes two values if we include the background in the training set -- otherwise $k$ takes one value. Alan thinks that Ju is minimizing the first tern with respect to $P$ and w.r.t $\theta$ -- so the $F$'s change. Then fixes $P$ and minimizes the third term with respect to $O$ (at least approximately) and $\theta$. If so the values of $\alpha, \beta, \theta$ do not matter.}
where $V_{ij},V_{ik} \in \{0, 1\}$ denotes the ground truth mask annotation in a format whether pixel $i$ belongs the corresponding part $j$ and object $k$. $\mathrm{Dis}$ is a distance function for measuring the similarity between pixel feature vector $\mathbf{F} \in \mathbb{R}^{HW\times D}$ and part feature embedding $\mathbf{P}\in \mathbb{R}^{N\times D}$ and object feature embedding $\mathbf{O}\in \mathbb{R}^{M\times D}$, where $N$, $M$ refers to the number of parts, objects, and $D$ is the embedding dimension and $\theta$ the learnable parameters in model. Note that $\sum_kV_{ik}=1$ as each pixel is assigned to one object (or background). In short, the problem has been transferred to learning good feature representations for pixels, parts and objects, which can then be used to perform clustering and compositing for segmentation problem.

This formulation can also easily gives mask prediction during inference. Distances between pixel feature and the feature centroids of parts or objects are firstly computed. Afterwards, pixels are assigned to the centroid with highest similarity:


\begin{align}
    {V}^{\dag}_{ij} = \mathrm{Dis}(\mathbf{F}_{i}, \mathbf{P}_{j})&,~{V}^{\ddag}_{ik} = \mathrm{Dis}(\mathbf{F}_{i}, \mathbf{O}_{k}), \\
    \hat{V}_{ij} = 
    \begin{cases}
        1, &\mathrm{if} ~ {V}^{\dag}_{ij} = \mathrm{max}({V}^{\dag}_{i*}) \\
        0, &\mathrm{otherwise}                    
    \end{cases}&,~\tilde{V}_{ik} = 
    \begin{cases}
        1, &\mathrm{if} ~ {V}^{\ddag}_{ik} = \mathrm{max}({V}^{\ddag}_{i*}) \\
        0, &\mathrm{otherwise}                    
    \end{cases}
    \label{formula:pred}
\end{align}
\alan{These equations say how we estimate $P$. Alan hopes that these are optimizing the first term of equation (3).}
where ${V}^{\dag}_{ij}, {V}^{\ddag}_{ik}$ are distance measurement from pixel $i$ to part $j$ and object $k$, and $\hat{V}_{ij},\tilde{V}_{ik} \in \{0, 1\}$ denotes the part and object mask prediction in a clustering assignment format. It is easy to see that an ideal case is that all pixels belonging to the same object share a similar feature vector, so that they will all be clustered to the corresponding part/object feature centroid.
These formulations also generalizes to per-pixel prediction case, where the parameters of last linear layer can be regarded as the feature centroids of the target classes. For mask classification case, the object queries can be interpreted as feature centroids for target objects.
Therefore, the problem of segmentation can be transferred as learning a feature vector as a centroid that can group corresponding pixels in a clustering manner.

\subsection{Compositor: Hierarchical Segmentation from Part to Whole}

In prior arts, objects are usually directly derived from pixels while an interpretable intermediate representation is missing. Though~\cite{he2021partimagenet} proposes a task to handle object parsing and object segmentation at the same time, object parsing is only used as a deep supervision to help the object segmentation. Nonetheless, we note that this strategy actually does not make full use of the great potential and relationship of the two tasks. Therefore, we introduce a bottom-up representation, consisting of pixels, parts, and objects, to better represent the two tasks. This representation further motivates us to propose Compositor, which groups pixels into semantic parts first, and then composites them into objects.

\textbf{Pixel embedding}. Given an image $\mathbf{I} \in \mathbb{R}^{H \times W \times 3}$, we use a CNN or Transformer backbone to extract the image features, which are then fed into a FPN~\cite{lin2017feature} to obtain the enhanced feature embedding. We further add it with a learnable positional encoding and forward it into a MLP layer to obtain the final feature embedding $\mathbf{F} \in \mathbb{R}^{HW\times D}$ for pixels.

\textbf{Part embedding}. Part is a natural intermediate representation for objects~\cite{kortylewski2020compositional}. Following Eq.~\ref{formula:opt_goal}, we consider a feature embedding $\mathbf{P} \in \mathbb{R}^{N\times D}$ for object parts with N specifying the number of parts, which groups pixels belonging to the same part region. Specifically, we initialize the part-level embedding with a set of learnable parameters, which are then updated to be the feature centroid of pixels belonging to the part. 

\textbf{Object embedding}. Object offers a higher level abstraction of the scene and is usually the most important notion that we care in the scene. Similar to parts, a feature vector $\mathbf{O} \in \mathbb{R}^{M\times D}$ is used to group pixels into object masks.

\textbf{Grouping Pixels into Parts.} As aforementioned, we aim to obtain a feature vector as part embedding, which can be used as a feature centroid and groups corresponding pixels. Inspired by k-means clustering algorithm, we firstly compute the affinity between part queries and pixels (\ie, $\mathbf{P} \times \mathbf{F}^T$), then we generate a soft assignment $\mathbf{W}\in \mathbb{R}^{N\times HW}$ from pixel embeddings to part embeddings by conducting $\mathrm{softmax}$ activation on part queries dimension followed by normalization. This soft assignment is then used as weights to average pixel embeddings to update part embeddings. Formally, we have:
\begin{align}
    % & \mathbf{W} = \mathop{\mathrm{softmax}}\limits_{N}(\mathbf{P}\times \mathbf{F}^T)
    & \mathbf{W}_{ji} = \frac{e^{\mathbf{P}_j\times (\mathbf{F}_i)^T}}{\sum_{k=1}^{N}e^{\mathbf{P}_k\times (\mathbf{F}_i)^T}} \\
    & \hat{\mathbf{P}}_j = \sum_{x=1}^{HW}(\frac{\mathbf{W}_{jx}}{\sum_{i=1}^{HW}\mathbf{W}_{ji}} \times \mathbf{F}_x)
    % & \hat{\mathbf{P}}_j =  \frac{\mathbf{W}_j}{\sum\nolimits_{i=1}^{HW}\mathbf{W}_{ji}} \times \mathbf{F},
    \label{formula:part_update1}
\end{align}
where $\hat{\mathbf{P}}_j \in \mathbb{R}^{1\times D}$ is the updated version of part embedding $\mathbf{P}$. We use the underscript $N$ and $HW$ to represent the axis for $\mathrm{softmax}$ and $\mathrm{sum}$ operation respectively. Inspired by the recent success and advanced architecture designs in Transformers, we further utilize a skip-connection for the embedding update and linear projections (denoted by $\mathrm{Linear}$) on feature vectors before the affinity is computed, which leads to a pixel-to-part clustering module:
\begin{align}
    & \mathbf{W}_{ji} = \frac{e^{\mathrm{Linear}(\mathbf{P}_j)\times (\mathrm{Linear}(\mathbf{F}_i))^T}}{\sum_{k=1}^{N}e^{\mathrm{Linear}(\mathbf{P}_k)\times (\mathrm{Linear}(\mathbf{F}_i))^T}} \\
    & \hat{\mathbf{P}}_j = \mathbf{P}_j + \sum_{x=1}^{HW}(\frac{\mathbf{W}_{jx}}{\sum_{i=1}^{HW}\mathbf{W}_{ji}} \times \mathrm{Linear}(\mathbf{F}_x))
\end{align}

\textbf{Compositing Parts into Objects.} 
% Similarly, we update the object embeddings through part embeddings in a soft k-means manner. 
Nonetheless, unlike pixels to parts where each pixel will eventually correspond to some part embeddings, the part embeddings may not all be used to obtain the object embedding (\eg, we may predict 50 parts embeddings while maybe only 5 corresponds to the target object.). To this end, part to object is more like compositing instead of clustering, where each part may be activated or dropped for the target object. Therefore, we propose to use $\mathrm{sigmoid}$ to transfer the affinity logits to weights for retrieving k-means update process. Besides, we also filter out those unactivated parts (based on the classification prediction) beforehand to ease the compositing process:
\begin{align}
    & \mathbf{W}_{kj} = \frac{1}{1+e^{-(\mathrm{Linear}(\mathbf{O}_k)\times (\mathrm{Linear}(\mathbf{A}_j))^T)}} \\
    & \hat{\mathbf{O}}_k = \mathbf{O}_k + \sum_{y=1}^{N}(\frac{\mathbf{W}_{ky}}{\sum_{j=1}^{N}\mathbf{W}_{kj}} \times \mathrm{Linear}(\mathbf{A}_y)) \\
    & \mathbf{A} = \{\mathbf{P}_j|\text{ if $\mathbf{P}_j$ is activated}\}.
    \label{formula:object_update}
\end{align}
\alan{This update may be equivalent to minimizing the third term in equation (3) with respect to $O$ but keeping $P$ fixed. Except we don't know $V_{jk}$. }

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/main_v10.pdf}
    \caption{Overview of the proposed framework Compositor, which clusters pixel embedding to part embedding and further composites part embedding to obtain object embedding. Part embedding and object embedding will be iteratively updated, and will be used to predict part/object categories and segmentation maps. }
    \label{fig:framework}
\end{figure*}

\subsection{Model Instantiation}
With the problem formulation as feature centroid learning and updating rules, we propose Compositor, which resolves the object segmentation problem in a hierarchical manner, by clustering pixel embedding into part embedding and then compositing part embedding into object embedding, which is then used to groups pixels and leads to object mask. As a result, Compositor is capable of handling semantic part segmentation, object segmentation and object classification simultaneously.

\textbf{Meta Architecture}. As illustrated in Figure \ref{fig:framework}, our meta architecture contains the following key components: an ImageNet pre-trained backbone (\eg, ResNet-50) with FPN for extracting multi-level pixel embedding from images, a pixel-to-part module for generating part embedding through clustering pixel embedding, a part-to-object module for obtaining object embedding through compositing part embedding and the prediction heads for transferring the updated embedding into final predictions.
% \qihang{@ju, refer and illustrate Fig 1. No need to refer maskformer, just describe ours. The details such as using final high-res feature can be placed in experiments/implementation details instead of here.}

\textbf{Training}. Inspired by previous works~\cite{carion2020end,wang2021max}, a matching process between predicted masks and ground truth segmentation masks is required for computing the loss. Following prior work \cite{stewart2016end}, Hungarian matching strategy is adopted for efficiently computing the matched pairs between prediction and ground-truth with the Hungarian algorithm.
After obtaining all matched pairs, we compute the loss between each of them as $\mathcal{L} = \lambda_{ce}\mathcal{L}_{ce} + \lambda_{dice}\mathcal{L}_{dice} + \lambda_{cls}\mathcal{L}_{cls}$, where $\mathcal{L}_{ce}$ and $\mathcal{L}_{dice}$ compute the binary cross-entropy loss and dice loss \cite{milletari2016v} for mask and $\mathcal{L}_{cls}$ computes the classification loss. $\lambda_{ce}, \lambda_{dice}, \lambda_{cls}$ sets the loss weight respectively. Our final loss consist of loss on parts and objects and can thus be formulated as:  
\begin{equation}
\begin{aligned}
    \mathcal{L} &= \lambda_{ce}\mathcal{L}_{ce_p} + \lambda_{dice}\mathcal{L}_{dice_p} + \lambda_{cls}\mathcal{L}_{cls_p} \\ &+ \beta(\lambda_{ce}\mathcal{L}_{ce_o} + \lambda_{dice}\mathcal{L}_{dice_o} + \lambda_{cls}\mathcal{L}_{cls_o}),
\end{aligned}
\end{equation}
where the subscript denotes parts and objects respectively and $\beta$ is an additional hyper-parameter for controlling the tendency to whether parts or objects of the model.

\textbf{Testing}. During inference, we obtain our final prediction through two $\mathrm{argmax}$ operations~\cite{wang2021max} to obtain the per-pixel mask and class predictions. We evaluate model performance with the metric mIoU \cite{everingham2015pascal} (\ie mean Intersection-over-Union) and mACC (\ie mean Accuracy) for parts and objects separately. 
% \qihang{is there anything special in inference? If not, we can introduce the evaluation metrics here.}

\textbf{Post-processing.} Ideally, for several categories of objects, each of their corresponding parts should be connected to at least one other object part. We exploit this weak object knowledge prior as a post-processing protocol to effectively remove portions of false part predictions on background. To be specific, during inference time, we search our predicted segmentation mask to find all connected components. We then go over all the components to check if they are connected to other parts and change the label of those isolated ones into background.

%With the introduced key ideas, we design a novel architecture TBD for handling semantic part segmentation, object segmentation and object classification simultaneously, where we first obtain a good part-level embedding through clustering per-pixel image features and then gradually integrates them to form the object-level embedding. Herein we introduce the detailed implementation of the TBD.

% \qihang{contents below should be removed, keep them now as reference.}
% We adopt the recent proposed meta architecture \cite{cheng2021per, cheng2021masked} as the base structure of our pipeline. As shown in Fig. \ref{TBD}, our meta architecture contains three main components: pixel encoder, pixel decoder, and TBD module. The pixel encoder extracts the pixel features either by a CNN or a Transformer backbone while the pixel decoder further enhances the extracted pixel features at different scales. Both the pixel encoder and pixel decoder are compatible with any existing designs. In the end, the TBD module takes the decoded pixel features as input and first update the part queries followed by learning the object queries.

% Note that we construct a series of TBD modules in order to handle the multi-scale pixel features input extracted from the pixel decoder, where they are feed into in a round robin fashion. The final out of the TBD decoder is the well-learned part queries $\mathbf{P}$ and object queries $\mathbf{O}$, which will further (1) multiply with the pixel features $\mathbf{F}$ to generate the predicted masks, and (2) generate corresponding class predictions for each mask by using Feed-Forward Network (FFN).

% \textbf{Loss functions}. Our training loss functions mostly follow the setting of Mask2Former \cite{cheng2021masked}. Both binary cross-entropy loss and the dice loss \cite{milletari2016v} are used for the mask prediction. The final loss furthers combines the classification loss of the mask. Formally speaking:
% \begin{align}
%     \mathcal{L} = \lambda_{ce}\mathcal{L}_{ce_p} + \lambda_{dice}\mathcal{L}_{dice_p} + \lambda_{cls}\mathcal{L}_{cls_p} + \beta(\lambda_{ce}\mathcal{L}_{ce_o} + \lambda_{dice}\mathcal{L}_{dice_o} + \lambda_{cls}\mathcal{L}_{cls_o}).
% \end{align}
% where $\lambda_{ce}, \lambda_{dice}, \lambda_{cls}$ stand for the loss weight of the three losses respectively and $\beta$ is an additional parameter for controlling the tendency to either parts or objects of the model.
